Photorealistic Text-to-Image Diffusion Models with Deep Language Understanding

We present Imagen, a text-to-image diffusion model with an unprecedented degree of photorealism and a deep level of language understanding. Imagen builds on the power of large transformer language models in understanding text and hinges on the strength of diffusion models in high-fidelity image generation. Our key discovery is that generic large language models (e.g. T5), pretrained on text-only corpora, are surprisingly effective at encoding text for image synthesis: increasing the size of the language model in Imagen boosts both sample fidelity and image-text alignment much more than increasing the size of the image diffusion model. Imagen achieves a new state-of-the-art FID score of 7.27 on the COCO dataset, without ever training on COCO, and human raters find Imagen samples to be on par with the COCO data itself in image-text alignment. To assess text-to-image models in greater depth, we introduce DrawBench, a comprehensive and challenging benchmark for text-to-image models. With DrawBench, we compare Imagen with recent methods including VQ-GAN+CLIP, Latent Diffusion Models, and DALL-E 2, and find that human raters prefer Imagen over other models in side-by-side comparisons, both in terms of sample quality and image-text alignment. See https://imagen.research.google/ for an overview of the results.

==> checklist.tex <==

\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:limitations}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{We describe the license of the public data we use in  Section~\ref{sec:limitations}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include  \benchmarkname prompts in the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We discuss the lack of consent from data subjects in web-scraped data in Section~\ref{sec:limitations}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Section~\ref{sec:limitations}.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{}
\end{enumerate}


\end{enumerate}

==> experiments_evaluationdetails.tex <==
\subsection{Evaluation Details}
\label{sec:experiments_evaluationdetails}

MS-COCO is a standard evaluation set used in existing text-to-image works \cite{ramesh-dalle,xu-cvpr-2018,nichol-glide}. Hence, we perform majority of comparisons and ablation studies on MS-COCO. We also compare \name with recent works \cite{ramesh-dalle2, crowson2022vqgan, rombach-cvpr-2022} on our proposed benchmark \benchmarkname.

We evaluate both image quality and image-text alignment across several metrics; we use automated metrics as well as human evaluation. For automated metrics, we use FID score \cite{heusel2017gans} to evaluate the fidelity of the samples, and CLIP score \cite{hessel2021clipscore, radford2021learning} to measure the alignment between the generated image and input text prompt. FID score compares the distribution of Inception features between the generated samples and the reference images, with a lower FID score generally corresponding to higher fidelity. CLIP score measures the dot product between the encoded reference text and the generated image, a higher CLIP score would generally imply better alignment under the CLIP model. Since guidance weight is an important knob to control image quality and text alignment, we report most of our ablation results using trade-off curves between CLIP and FID scores across a range of guidance weights. Both metrics have limitations, for example FID is not fully aligned with perceptual quality \cite{parmar-cvpr-2022}, and CLIP is unable to perform counting well \cite{radford2021learning}. Due to these limitations, we also use human evaluation to assess for image quality, and caption similarity. 

To assess the image quality on MS-COCO, we run a 2-alternative forced choice (2AFC) evaluation where the rater is asked to choose between the model generation and the reference image based on the question: ``Which image is more photorealistic (looks more real)?''. Note that this set up is different from that of \benchmarkname, which does not have reference images. We report the percentage of times raters choose model's generations over reference images (a.k.a. the \emph{preference rate}). A 50\% preference rate implies the evaluator has equal preference between the model's samples vs. the reference.

For image-text alignment, human raters are shown a model-generated image (or a reference image) together with the input caption, and asked ``Does the caption accurately describe the above image?''. The raters are allowed to choose among three possible options : ``yes'', ``somewhat'', ``no'', each corresponding to scores of 100, 50, and 0, respectively. This was done independently for both model samples and the reference images. We report both values (e.g., the reference image may not be well aligned with the corresponding caption in certain cases). We also report evaluation results on a filtered set of examples, i.e. examples from the reference that do not contain any person in it. We filter based on a set of people-specific identifiers in text prompts.

For both types of human evaluations, we use 200 randomly chosen (image, caption) pairs from the MS-COCO test set, and ran the human survey in four batches each containing 50 images. We obtained total of 100 responses for each of 200 captions.
Before we aggregate the responses, we interleave 10 ``control'' questions and only count responses from raters who correctly rated at least 80\% of the control questions. After this filtering, we had at least 73 and 51 ratings per image for image quality and image-text alignment evaluations, respectively.



==> limitations.tex <==



